One-shot Unsupervised Domain Adaptation with Personalized Diffusion Models

Adapting a segmentation model from a labeled source domain to a target domain, where a single unlabeled datum is available, is one the most challenging problems in domain adaptation and is otherwise known as one-shot unsupervised domain adaptation (OSUDA). Most of the prior works have addressed the problem by relying on style transfer techniques, where the source images are stylized to have the appearance of the target domain. Departing from the common notion of transferring only the target ``texture'' information, we leverage text-to-image diffusion models (e.g., Stable Diffusion) to generate a synthetic target dataset with photo-realistic images that not only faithfully depict the style of the target domain, but are also characterized by novel scenes in diverse contexts. The text interface in our method Data AugmenTation with diffUsion Models (DATUM) endows us with the possibility of guiding the generation of images towards desired semantic concepts while respecting the original spatial context of a single training image, which is not possible in existing OSUDA methods. Extensive experiments on standard benchmarks show that our DATUM surpasses the state-of-the-art OSUDA methods by up to +7.1%. The implementation is available at https://github.com/yasserben/DATUM

==> tables/ablation/ablation_1.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX. \sub{@Yasser, please fill the values indicated in red. Please use blue color so that I will know when you have filled them.}}\label{tab: }
\scriptsize
\begin{tabular}{lrrrr}\toprule
\textbf{number of shots} &\textbf{training steps} &\textbf{mIoU} & FID\\\midrule
\multirow{5}{*}{1} &200 &57.21 & \doubt{112.8} \\
&400 &55.23 & \doubt{94.6}\\
&600 &53.87 & \doubt{100.1}\\
&800 &50.82 & \doubt{116.0}\\
&1000 &52.76 & \doubt{111.7}\\
\hline
\multirow{5}{*}{5} &200 &54.07 & \doubt{fill}\\
&400 &\doubt{55.76} & \doubt{87.5}\\
&600 &57.72 & \doubt{75.5}\\
&800 &54.79 & \doubt{74.3}\\
&1000 &\doubt{53.77} & \doubt{89.2}\\
\hline
\multirow{5}{*}{10} &200 &56.57 & \doubt{109.6}\\
&400 &55.27 & \doubt{116.2}\\
&600 &55.52 & \doubt{113.9}\\
&800 &54.86 & \doubt{92.3}\\
&1000 &56.51 & \doubt{91.4}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/ablation/ablation_2.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Effect of training steps}\label{tab: }
%\scriptsize
\begin{tabular}{lrrrr}\toprule
Method &train. steps &mIoU &FID \\\midrule
Stable Diffusion &0 &52.4 & \doubt{181.8}\\
\textbf{\method} &\textbf{200} &\textbf{57.2} & \doubt{112.8} \\
\method &400 &55.2 & \doubt{94.6} \\
\method &600 &53.9 & \doubt{100.1} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/ablation/ablation_4.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Impact of the size of the target domain}\label{tab: }
\scriptsize
\begin{tabular}{lrrr}\toprule
\textbf{Method} &\textbf{size target domain} &\textbf{mIoU} \\\midrule
\multirow{5}{*}{\textbf{DAFormer}} &10 &55.0\% \\
&50 &58.2\% \\
&100 &61.8\% \\
&1000 &62.6\% \\
&2975 &68.3\% \\
\multirow{5}{*}{\textbf{DAFormer+Ours}} &10 &50.6\% \\
&50 &52.8\% \\
&100 &54.5\% \\
&1000 &57.2\% \\
&2975 &57.2\% \\
\bottomrule
\end{tabular}
\end{table}

==> tables/ablation/ablation_5.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{type of target domain}\label{tab: }
\scriptsize
\begin{tabular}{lrr}\toprule
\textbf{target domain} &\textbf{mIoU} \\\midrule
Stylized using RAIN module &53.43\% \\
Generated using Dreambooth &57.21\% \\
\bottomrule
\end{tabular}
\end{table}
